Survey on Plagiarism Detection in Large Language Models: The Impact of ChatGPT and Gemini on Academic Integrity

The rise of Large Language Models (LLMs) such as ChatGPT and Gemini has posed new challenges for the academic community. With the help of these models, students can easily complete their assignments and exams, while educators struggle to detect AI-generated content. This has led to a surge in academic misconduct, as students present work generated by LLMs as their own, without putting in the effort required for learning. As AI tools become more advanced and produce increasingly human-like text, detecting such content becomes more challenging. This development has significantly impacted the academic world, where many educators are finding it difficult to adapt their assessment methods to this challenge. This research first demonstrates how LLMs have increased academic dishonesty, and then reviews state-of-the-art solutions for academic plagiarism in detail. A survey of datasets, algorithms, tools, and evasion strategies for plagiarism detection has been conducted, focusing on how LLMs and AI-generated content (AIGC) detection have affected this area. The survey aims to identify the gaps in existing solutions. Lastly, potential long-term solutions are presented to address the issue of academic plagiarism using LLMs based on AI tools and educational approaches in an ever-changing world.

==> comments.tex <==
% \author{
%     Shushanta Pudasaini \\
%     Technological University Dublin \\
%     Dublin \\
%     \texttt{\{Shushanta Pudasaini\}shushanta574@gmail.com}\\
%     \And
%     Luis Miralles \\
%     Technological University Dublin \\
%     Dublin \\
%     \texttt{\{Luis Miralles\}Luis.Miralles@tudublin.ie}\\
%     \And
%     Marisa Llorens Salvador \\
%     Technological University Dublin \\
%     Dublin \\
%     \texttt{\{Marisa Llorens Salvador\}marisa.llorens@tudublin.ie}\\
    
% }

% The capabilities of recent LLMs are unparalleled. 
% LLMs are deep learning-based models built to perform a variety of Natural Language Processing (NLP) tasks. Brainstorming, generating counterarguments, summaries, and abstracts, and correcting grammar are a few of the NLP tasks, that LLMs are capable of. 

% \author{
%   Shushanta Pudasaini \\
%   Technological University Dublin \\
%   % Univ \\
%   Dublin\\
%   \texttt{shushanta574@gmail.com} \\
%   %% examples of more authors
%    \AND
%   Marisa Llorens Salvador \\
%   Technological University Dublin \\
%   Dublin \\
%   \texttt{marisa.llorens@tudublin.ie} \\
%    \And
%   Luis Miralles \\
%   % Affiliation \\
%   Technological University Dublin \\
%   Dublin\\
%   \texttt{Luis.Miralles@tudublin.ie} \\

  %% \And
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
  %% \And
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\




% This paper examines recent tools and algorithms developed to detect AI-generated text as well as identifies the limitations of existing solutions. 

% Since the eruption of ChatGPT, students can complete their assignments and exams, and researchers can generate academic content for publishing due to which academic cheating has increased. This has led to problems such as students not learning because of dependency on such tools and researchers not publishing authentic content. Lecturers and publishers have no idea how to detect such AI-generated content. With the power of Generative AI tools increasing day by day resulting generation of even more human-like text, the detection of such text has been even more challenging. This has taken the academic world by storm. In this research, we study the recent tools and algorithms developed for the detection of such AI-generated text. We aim to identify the gaps in the existing solutions for the problem and propose potential solutions based on the gaps identified.

% The emergence of ChatGPT and other generative AI tools has created a new challenge for academia. Students can now utilize these tools to complete assignments and exams, while researchers can potentially generate content for publication. This has led to a rise in academic dishonesty, with students potentially forgoing learning due to a reliance on such tools and researchers potentially publishing content that lacks authenticity. Lecturers and publishers currently lack effective methods to detect AI-generated content. As the capabilities of generative AI tools continue to grow, producing even more human-like text, the detection of such content becomes increasingly challenging. This development has significantly impacted the academic world. In this research, we will examine recent tools and algorithms developed to detect AI-generated text. We aim to identify limitations in existing solutions and propose potential solutions based on these gaps.



% 1) Students are using Large Language Models (LLM) such as ChatGPT and BARD for assignment writing which has questioned the originality of the student's work. \textbf{Explain why is bad that students use LLM.} 2) Some detection mechanisms in the literature have been used during the years. 3) Traditional methods do not work well for detecting AI-generated text. (It can be interesting to say why detecting plagiarism is so difficult) 4) In this research we analyze the gaps and limitations of current systems. 5) We also draft solutions to address the problem of students using AI to do their work. 6) We finally write the solutions to the problems.

% This research focuses on several aspects of using large language models in academia. The potential use of these models and the impact of their use on originality have been discussed. Likewise, the algorithms developed to solve the issue of academic theft have been surveyed and the state-of-the-art techniques have been tested with different attacking techniques such as recursive paraphrasing. Apart from the open source Artificial Intelligence Generated Content (AIGC) detection algorithms, the commercial AIGC detection tools have been tested with the attacking techniques. Finally, the paper discusses whether the top AIGC detection and algorithms tools can be relied upon or not and the possible alternatives for the evaluation of academic works.



% About forty-nine thousand text generation models have been open-sourced in the largest platform for sharing NLP models called HugginFace which suggests that these LLMs are about to grow with more and more capabilities.



% LLMs like ChatGPT are mostly used for writing assignments and research by college students \cite{tossell2024student}.

% ChatGPT now being the fastest growing technology in the world, LLMs like ChatGPT have started to show potential in changing how automation can be introduced in every industry \cite{forbesChatGPTFastest}. From students using ChatGPT for essay writing \cite{ymerdigital} to researchers using it for research paper writing\cite{nihChatGPTAcademic}, these LLMs have disrupted the academic industry by raising serious doubts about maintaining originality in academic settings \cite{sciencedirectChatGPTAcademia}.


 
% Alongside this, a survey of different evasion techniques developed to fool such tools identifies gaps in the existing solutions. Based on the survey and the gaps identified, we propose different technical solutions and alternative educational solutions in section 6. 

% The major contributions of the research are listed below.
% \begin{itemize}
%     \item Extensive survey of tools and techniques used for academic misconduct
%     \item Extensive survey of AIGC detection algorithms 
%     \item Extensive survey of AIGC detection evasion tools and techniques
%     \item Proposing potential solutions to academic misconduct
% \end{itemize}



% \textbf{Contributions of the paper} \\
% In this paragraph following contributions of the research are discussed:
% \begin{itemize}
%     \item research on academic misconduct
%     \item survey of tools used for academic misconduct
%     \item survey on AIGC detection algorithms and tools
%     \item research on the efficiency of AIGC detection tools
%     \item finding out AIGC evasion techniques
%     \item discussion of the possibility of AIGC detection
%     \item putting forward a new method of AIGC detection
% \end{itemize}

% \section{Academic Misconduct and plagiarism}
% This section will be mostly focused on the state-of-the-art tools, algorithms for generating text, AIGC detection, and techniques for evading AIGC detection tools

% \textit{\textbf{I believe that the paper's main theme is to prepare a literature survey on Academic misconduct focusing on AIGC detection being the most recent, frequent one in today's circumstances.}}


% \subsection{Pointing out the major problem statement::Types of Academic Misconduct - Especially focused on AI-generated plagiarism}
% \begin{itemize}
%     \item Discuss several ways of performing academic misconduct such as

%     \begin{itemize}
%         \item Academic misconduct utilizing others' information by simply claiming others' work, using paraphrasing tools, and causing plagiarism
%         \item Academic misconduct utilizing others' code to submit programming assignments either using entirely or by modification.
%         \item Academic misconduct using the generative AI tools for text and code both
%     \end{itemize}    
% \end{itemize}

% \textbf{Point out that AIGC misconduct is now the most frequently used one and requires high concerns which state the major problem we are trying to solve/discuss}


% The different ways LLMs have been raising problems for academia are represented in Figure \ref{fig: LLMs usecases}. 


% \begin{figure}[hbt!]
%     \centering
%     \includegraphics[width=0.6\textwidth,height=\textheight,keepaspectratio]{LLM_USECASES.png}
%     \caption{Different ways LLMs can be used for Academic Misconduct.}
%     \label{fig: LLMs usecases}
% \end{figure}



% With the advancement of Generative AI tools and algorithms, there are several issues and complications brought by these tools. 

% \textcolor{purple}{Ask questions on whether other issues should be discussed or not.}



% \subsection{Giving background of the problem: Everything about LLMs-How they can be used and what are they expected to do in the future}

% \textit{\textbf{I want to discuss here how the AIGC arose, why it is getting more difficult to solve the problem of AIGC detection and what the problems caused by AIGC conveying why the problem we are discussing is highly critical and difficult to solve at the same time}}

% \textbf{1st paragraph: Generative AI, its rise and scopes}
% \begin{itemize}
%     \item 2-3 sentences on generative AI and how generative AI has been influencing the internet and daily lives
%     \item About various types of generative AI tools such as ChatGPT, BARD, DALLE and multimodal GEN AI such as GPT-4 and Gemini
%     \item different scopes of usage of Gen AI tools such as problem-solving, generating new contents
    
% \end{itemize}

% \textbf{2nd paragraph: AIGC and types of AIGC}
% \begin{itemize}
%     \item about AI-generated content and stats on the proportion of AIGC on the internet nowadays
%     \item types of AIGC: text, code, image, and audio and stating that this research mainly focuses on text AIGC
    
% \end{itemize}

% \textbf{3rd paragraph: SOTA algorithms for text generation}
% \begin{itemize}
%     \item point out that OPENAI GPT-4 and Google Gemini model are the SOTA algorithms for text generation
%     \item briefly discusses how such efficient text generation was achieved by using the Reinforcement Learning Human Feedback (RLHF) algorithm implemented on the decoder-based transformer architecture on previous GPT models. Start from basic n-gram language models being used for text generation
% \end{itemize}

% \textbf{Discuss how LLMs are getting better day by day which makes the problem even more difficult}


% \textcolor{red}{Figure of a curve of no of parameters in LLMs vs year demonstrating that LLMS are getting better}

% % \clearpage

% \textbf{4th paragraph: Problems caused by AIGC}
% \begin{itemize}
%     \item discusses the problems caused by AIGC such as misinformation due to hallucinations, fraudulent activities, bias and ethical considerations, energy consumption due to Gen AI
%     \item brief discussion on academic misconduct being one of the major problems created by Gen AI tools    
% \end{itemize}

% \textcolor{red}{Figure pointing out the major problems caused by LLMs}
% \begin{figure}[hbt!]
%     \centering
%     \includegraphics[width=200mm]{Threats of AIGC.png}
%     \caption{Problems Caused by AIGC}
%     \label{fig: Problems caused by AIGC}
% \end{figure}

% \textbf{5th paragraph: Types of Academic Misconduct}

% \section{Solutions to Academic Misconduct}
% \textbf{1st paragraph: Solutions to Academic Misconduct}
% \begin{itemize}
%     \item starting from traditional plagiarism algorithms
%     \item discussion on PAN series of scientific events and shared tasks on digital text forensics and stylometry
%     \item discussing the efficiency of plag checking tools like Turnitin and its use in most of the universities and research conferences.
%     \item introduction of paraphrasing algorithms and tools like Quillbot disrupting the harmony of academic fairness
%     \item discussing how plagiarism and academic misconduct were more frequent and easy with the introduction of ChatGPT using some statistics 
%     \item discussing the need and rise of AIGC detection with major landmark by OpenAI text detector from OpenAI itself
%     \item discussing how AIGC evasion techniques have also risen
    
% \end{itemize}


% \begin{table}[htbp]
%   \centering
%   \caption{Table representing Google Scholar search results on the term "Plagiarism Detection"}
%   \begin{tabular}{|c|c|}
%   \toprule
%     Year Range  & Number of Search Results \\
%     \midrule
%     1980 - 1990  & 583 \\
%     1990 - 2000  & 831 \\
%     2000 - 2010 & 5750 \\
%     2010 - 2020 & 16900 \\
%     2020 - 2024 & 14700 \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}[htbp]
%   \centering
%   \caption{Table representing Google Scholar search results on the term "Plagiarism Detection"}
%   \begin{tabular}{|c|c|}
%   \toprule
%     Year Range  & Number of Search Results \\
%     \midrule
%     1980 - 1990  & 583 \\
%     1990 - 2000  & 831 \\
%     2000 - 2010 & 5750 \\
%     2010 - 2020 & 16900 \\
%     2020 - 2024 & 14700 \\
%     \bottomrule
%   \end{tabular}
% \end{table}



% With such a combined technique, students can easily generate text that cannot be detected by plagiarism detection and AIGC detection tools online which raises a question mark on the originality. 





% \section{Plagiarism techniques and their current limitations}

% \subsection{Plagiarism Detection}
% \textbf{1st paragraph: Types of plagiarism}
% \begin{itemize}
%     \item intrinsic and extrinsic
%     \item code and text plagiarism
%     \item character preserving, syntax preserving, semantics preserving, idea preserving plagiarism and ghostwriting
% \end{itemize}



% \textbf{2nd paragraph: Top plagiarism detection algorithms}
% \begin{itemize}
%     \item Top preprocessing techniques
%     \item top lexical detection methods with tabular representation
%     \item top syntax-based methods with tabular representation
%     \item top semantics-based methods with tabular representation
%     \item top idea-based method with tabular representation
%     \item Other methods like ensemble and mixed methods
% \end{itemize}

% \textcolor{green}{Table showing the open source datasets for plagiarism deteection}
% \textcolor{green}{Table showing top plagiarism detection algorithms}

% \textbf{3rd paragraph: Top plagiarism detection tools} \\
% \newline
% Comparison of top plagiarism detection tools such as Turnitin, Grammarly, CopyLeaks, Plagibot
% \newline

% \textcolor{green}{Table of survey on top plagiarism detection tools}

% \textbf{4th paragraph: Linking Plagiarism to AIGC detection}
% \begin{itemize}
%     \item starting from traditional plagiarism algorithms
%     \item discussion on PAN series of scientific events and shared tasks on digital text forensics and stylometry
%     \item discussing the efficiency of plag checking tools like Turnitin and its use in most of the universities and research conferences.
%     \item introduction of paraphrasing algorithms and tools like Quillbot disrupting the harmony of academic fairness
%     \item discussing how plagiarism and academic misconduct were more frequent and easy with the introduction of ChatGPT using some statistics 
%     \item discussing the need and rise of AIGC detection with major landmark by OpenAI text detector from OpenAI itself
% \end{itemize}


% An example of a paragraph written by a human along with a paragraph generated using ChatGPT describing the animal cow is shown in Fig \ref{fig:ChatGPTvshuman}. 




% \textbf{1st para: Demonstration} \\
% Demonstration on how dishonest academic content is being generated from AI and the use of LLMs for paraphrasing to escape plagiarism

% \textcolor{red}{Fig demonstrating how tools like ChatGPT are being used as paraphrasers on others' content resulting in plagiarism }


% \textbf{2nd para: AIGC text vs human written text} \\
% Show an example of AIGC text and human-written text. Discuss the common patterns of AIGC text like word repetitions, complex syntactic sentences, less personal details, and so on. Discuss how difficult is it for humans to differentiate and put data of human evaluators' efficiency conducted by other papers.

% \textcolor{red}{Figure showing an example of AIGC text and human written text on the same topic}


% \textbf{3rd para: AIGC Detection text datasets} \\
% In this paragraph, I intend to discuss different open-source datasets developed for AIGC detection. I am planning to write about the diversity, size, and methods of how they were developed. Ends with a table containing details about the dataset, publisher, number of training and testing observations, size, the domain of the dataset

% \textcolor{green}{Table showing the open source AIGC detection datasets}

% \textbf{4th para: Watermarking and Perplexity-based AIGC detection algorithms} //
% In this paragraph, I will discuss the watermarking-based and perplexity-based AIGC detection papers.

% \textcolor{green}{Table showing the recent Watermarking and Perplexity-based AIGC detection algorithms}


% \textbf{5th para: Training based AIGC detection algorithms} \\
% Starting with the OPENAI text detector, I will discuss most of the training-based classifiers for AIGC detection

% \textcolor{green}{Table showing the recent Training based AIGC detection algorithms}



% \textbf{6th para: Zero shot-based AIGC detection} \\
% Starting with DetectGPT, I will discuss most of the zero-shot-based AIGC detection algorithms here.

% \textcolor{green}{Table showing the recent Zero shot-based AIGC detection algorithms}

% \textbf{7th para: Top AIGC detection tools} \\
% Comparison of top AIGC detection tools such as Originality AI, Copyleaks, GPTZero
% \textcolor{green}{Table showing the open source and commercial AIGC detector tools available online}


% \section{Evaluation of Current Plagiarism and AIGC Detection Tools }

% As reported by Turnitin, over 16,000 academic institutions, publishers and corporations use the Turnitin software to prevent plagiarism \cite{turnitinTurnitinCelebrates}. However, 97\% of the institutions have not implemented any formal policy on using AI tools by students and 71\% of the instructors have never used AI writing tools  \cite{tytonpartners}. On the other hand, 51\% of the students responded to continue using generative AI tools even if prohibited by the institution \cite{tytonpartners}. A survey conducted among 1147 instructors reported that most of the instructors permitted the use of generative AI writing tools for brainstorming ideas for an assignment, helping edit writing and outlining a structure for an assignment whereas the instructors were against the use of generative AI writing tools for writing a small and large part of an assignment or even an entire assignment \cite{tytonpartners}. The data indicates that a formal policy on the usage of generative AI writing tools should be developed and regulated by every organization. Along with such a policy, an efficient and reliable tool which can detect AI-generated content is highly essential. Turnitin launched the AI writing detection tool on April 4, 2023, and since over 50 million submissions have been processed globally \cite{turnitinTurnitinCelebrates}. However, false positives have been acknowledged by Turnitin itself \cite{turnitinUnderstandingFalse}. 
% \subsection{Evasion Techniques }
% The major problem with protecting originality in academic settings is the new evasion techniques that people come up with existing plagiarism detection and AIGC detection tools. Ahmed M. Elkhatat et al. experimented with four of the most commonly used evasion techniques applied to top plagiarism detectors available online and found plagiarism detectors cannot detect simple evasion techniques \cite{elkhatat2021some}. The evasion techniques that students mostly use to fool existing online plagiarism detection tools and the result of checking those tools through every technique are presented in Table 10. 

% \begin{table}[htbp]
%     \centering
%     \caption{Comparison of Plagiarism Evasion Techniques and Detection Systems}
%     \label{tab:plagiarism_comparison}
%     \begin{tabular}{|l|p{5cm}|p{3.5cm}|p{3.5cm}|}
%          
%         \textbf{Evasion Technique} & \textbf{Description} & \color{green}\textbf{Successful Plagiarism Detectors} & \color{red}\textbf{Unsuccessful Plagiarism Detectors} \\  
%         Imaged Texts & Convert all text to image and export file as PDF & None & Turnitin, iThenticate, Copyscape, PlagAware, StrikePlagiarism.com, Unicheck, Check-For-Plag, Blackboard-SafeAssign \\  
%         Quoted & Insert invisible white quotation marks for all paragraphs & Blackboard-SafeAssign, Copyscape, PlagAware, StrikePlagiarism.com, Unicheck, Check-For-Plag & Turnitin, iThenticate, PlagScan \\  
%         Letter-like Symbols & Replace most common letters like a, e, o with their Latin small letter & Turnitin, iThenticate, PlagAware & Blackboard-SafeAssign, Copyscape, PlagScan, Unicheck, Check-For-Plag \\  
%         Invisible Letters & Replace spaces within words with any white color letter & StrikePlagiarism.com & Turnitin, iThenticate, Copyscape, PlagAware, Unicheck, Check-For-Plag, Blackboard-SafeAssign \\  
%     \end{tabular}
% \end{table}
% Similarly, with AI-generated text detection also attackers are coming up with several evasion techniques. These evaluation techniques vary with the solution applied for AIGC detection. For instance, for AIGC detection systems against watermarking, techniques such as watermark stealing \cite{jovanovic2024watermark}, Self Color Testing-based Substitution (SCTBS) \cite{wu2024bypassing}, and language translation \cite{he2024can} have been developed. Similarly, paraphrasing, word substitution, and sentence substitution are used to evade binary classification training-based AIGC detection models \cite{peng2024hidding} \cite{krishna2024paraphrasing}. Other most common evasion techniques used to fool AIGC detectors are prompting \cite{lu2023large}, adversarial attacks \cite{peng2024hidding}, single space adding technique \cite{cai2023evade} and reinforcement learning\cite{nicks2023language}. These evasion techniques are tested on different AIGC detection models and have been successful in fooling those models resulting in a high drop in AUC, and detection accuracy which is presented in Table 11.


% \begin{table}[htbp]
%   \centering
%   \caption{AIGC Detection Evasion Experiments and Results}
%     \begin{tabular}{|p{4.5cm}|p{4.5cm}|p{3.5cm}|p{3.5cm}|}
%     \toprule
%     \textbf{Experiment} & \textbf{Evasion Technique Applied} & \textbf{Tested Models} & \textbf{Results} \\
%     \midrule
%     Hiding the Ghostwriters: An Adversarial Evaluation of AI-Generated Student Essay Detection & Paraphrasing, Word Substitution, Sentence Substitution & ArguGPT, CheckGPT, RoBERTA-Single, RoBERTa-QA, Quality & Significant drop in accuracy and AUC on all models \\
%     Bypassing LLM Watermarks with Color-Aware Substitutions & Self Color Testing-based Substitution & Watermarked LLMs & SCTS evasion technique is highly effective for different watermarking schemes \\
%     Watermark Stealing in Large Language Models & Watermark Stealing & Watermarked LLMs & For under \$50 an attacker can both spoof and scrub state-of-the-art watermarking schemes with a success rate over 80\% \\
%     Paraphrasing evades detectors of AI-generated text, but retrieval is an effective defence & Paraphrasing, Word Substitution, Sentence Substitution & Watermarking, GPTZero, DetectGPT and OpenAI text Classifier & Paraphrasing dropped detection accuracy of DetectGPT from 70.3\% to 4.6\% \\
%     Large Language Models can be Guided to Evade AI-Generated Text Detection & Substitution-based In-Context example Optimization method (SICO) & GPT3-D, DPT2-D, GPTZero, OpenAI-D, DetectGPT, Log\_Rank & Decreased the AUC of six detectors by 0.5 on average \\
%     Language Model Detectors are easily optimized against & Reinforcement Learning & OpenAI RoBERTa-Large detector & Decreased the AUC of OpenAI detector from 0.84 to 0.62 \\
%     Stumbling Blocks: Stress Testing the Robustness of Machine-Generated Text Detectors Under Attacks & Editing, Paraphrasing, Prompting, and Co-generating & Watermark, OpenAI Detectors, GLTR, DetectGPT & Performance drops by 35\% across all attacks \\
%     Evade ChatGPT detectors via a single space & Add a single-space Space Strategy & ChatGPT, GPTZero, GPT-4 & increased the evasion rate close to 100\% \\
    
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%


% Thus, multiple research studies are ongoing for detecting fake academic content with plagiarism and AIGC detection. However, research studies on how these algorithms can be fooled with new evasion techniques have also been done. Along with this, Large Language Models (LLMs) have completely changed the game because of their potential and several use cases for performing academic misconduct. And they are becoming better day by day and producing even more human-like text. This circumstance raises the question of the feasibility of detecting such fake content. Thomas Lancaster shed light on how students can use ChatGPT to complete their assignments, and how watermarking solutions can be used to catch the students, giving better small-scale study results\cite{lancaster2023artificial}. However, he concludes that those watermarking solutions can not be relied upon to detect AI-generated content and alternative solutions should be developed encouraging the academia to work with such AI tools positively rather than against it \cite{lancaster2023artificial}. Sadasivan et al. demonstrated almost all AIGC detectors fail with recursive paraphrasing attacks \cite{sadasivan2023can}. 



% \section{Evaluation of Solutions to Avoid Academic Misconduct}
% \textbf{1st para: Current way of Evaluation} \\
% Discuss the fairness of the current way of evaluating new research articles and student submissions \\
% State that the current way of evaluation by checking plagiarism in paper submissions is only eradicating certain academic thefts but AIGC detection should also be prioritized \\

% \textbf{2nd para: Usage of LLMs by researchers and students}\\
% Stats on the usage of Generative AI platforms by students and researchers \\
% more powerful and large language models coming up with time \\
% Students are coming up with new AIGC detection evasion techniques \\

% \subsection{Plagiarism and AIGC Detection Evasion Techniques}
% \textbf{1st para: Are the plagiarism detection and AIGC detection models outdated?} \\
% Discussion on how efficient are plagiarism detection and AIGC detection models in production-level or real-time settings

% \textbf{2nd para: Plagiairism Evasion Techniques}
% Demonstrate how plagiarism evasion techniques such as paraphrasing from tools like Quilbot are fooling plagiarism checker tools like Turnitin

% \textbf{3rd para: AIGC Detection Evasion Techniques}
% Demonstrate how techniques such as space infiltration, sentence and word substitution are fooling top AIGC detectors like GPTZero

% \textbf{4th para: conclude that current AIGC detection and plagiarism detection models are outdated}






% \section{Discussion and Analysis}

% \subsection{Feasibility of solving the problem}
% \textbf{1st para: what should be prioritized? memory over problem-solving or individual skills over people skills}
% Discuss that universities should come up with testing students' problem-solving skills. 

% \textbf{2nd para: Feasibility of developing a new algorithm for AIGC detection}
% Discuss how current algorithms are failing to catch AIGC text. \\
% Discuss that instead of training binary classifiers for AIGC detection, other alternatives should be considered

% \subsection{Issues in Existing Solutions}
% \textit{\textbf{Here I intend to discuss that existing solutions are only binary based. Existing solutions consider the embeddings generated by the whole text rather than the gist of the textual content}}

% \subsection{Possible Solutions}

% \subsubsection{Unidirectional technical solution: Comparing idea or gist of given chunks of text rather than word by word or sentence by sentence}

% Current AIGC detectors are developed based on the embedding of the whole text \\
% The proposed solution compares whether the major gist or idea of the two documents matches or not. \\
% \clearpage



% % \clearpage

% \subsection{Bidirectional technical solutions}
% \textbf{Estimating the complexity and quality of paper rather than simple classification}


% \subsection{Alternative educational solution}
% \textbf{1st para: Changing the way of examinations}
% Focusing more on problem-solving examinations rather than memorizing


% \section{Conclusion}
% \label{sec:headings}

% \lipsum[4] See Section \ref{sec:headings}.

% \subsection{Headings: second level}
% \lipsum[5]
% \begin{equation}
% \xi _{ij}(t)=P(x_{t}=i,x_{t+1}=j|y,v,w;\theta)= {\frac {\alpha _{i}(t)a^{w_t}_{ij}\beta _{j}(t+1)b^{v_{t+1}}_{j}(y_{t+1})}{\sum _{i=1}^{N} \sum _{j=1}^{N} \alpha _{i}(t)a^{w_t}_{ij}\beta _{j}(t+1)b^{v_{t+1}}_{j}(y_{t+1})}}
% \end{equation}

% \subsubsection{Headings: third level}
% \lipsum[6]

% \paragraph{Paragraph}
% \lipsum[7]

% \section{Examples of citations, figures, tables, references}
% \label{sec:others}
% \lipsum[8] \cite{kour2014real,kour2014fast} and see \cite{hadash2018estimate}.

% The documentation for \verb+natbib+ may be found at
% \begin{center}
%   \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
% \end{center}
% Of note is the command \verb+\citet+, which produces citations
% appropriate for use in inline text.  For example,
% \begin{verbatim}
%    \citet{hasselmo} investigated\dots
% \end{verbatim}
% produces
% \begin{quote}
%   Hasselmo, et al.\ (1995) investigated\dots
% \end{quote}

% \begin{center}
%   \url{https://www.ctan.org/pkg/booktabs}
% \end{center}


% \subsection{Figures}
% \lipsum[10] 
% See Figure \ref{fig:fig1}. Here is how you add footnotes. \footnote{Sample of the first footnote.}
% \lipsum[11] 

% \begin{figure}
%   \centering
%   \fbox{\rule[-.5cm]{4cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{Sample figure caption.}
%   \label{fig:fig1}
% \end{figure}

% \subsection{Tables}
% \lipsum[12]
% See awesome Table~\ref{tab:table}.

% \begin{table}
%  \caption{Sample table title}
%   \centering
%   \begin{tabular}{lll}
%     \toprule
%     \multicolumn{2}{c}{Part}                   \\
%     \cmidrule(r){1-2}
%     Name     & Description     & Size ($\mu$m) \\
%     \midrule
%     Dendrite & Input terminal  & $\sim$100     \\
%     Axon     & Output terminal & $\sim$10      \\
%     Soma     & Cell body       & up to $10^6$  \\
%     \bottomrule
%   \end{tabular}
%   \label{tab:table}
% \end{table}

% \subsection{Lists}
% \begin{itemize}
% \item Lorem ipsum dolor sit amet
% \item consectetur adipiscing elit. 
% \item Aliquam dignissim blandit est, in dictum tortor gravida eget. In ac rutrum magna.
% \end{itemize}


% \section{Conclusion}
% Your conclusion here
